Bosehedral: Compiler Optimization for Bosonic Quantum Computing

Bosonic quantum computing, based on the infinite-dimensional qumodes, has shown promise for various practical applications that are classically hard. However, the lack of compiler optimizations has hindered its full potential. This paper introduces Bosehedral, an efficient compiler optimization framework for (Gaussian) Boson sampling on Bosonic quantum hardware. Bosehedral overcomes the challenge of handling infinite-dimensional qumode gate matrices by performing all its program analysis and optimizations at a higher algorithmic level, using a compact unitary matrix representation. It optimizes qumode gate decomposition and logical-to-physical qumode mapping, and introduces a tunable probabilistic gate dropout method. Overall, Bosehedral significantly improves the performance by accurately approximating the original program with much fewer gates. Our evaluation shows that Bosehedral can largely reduce the program size but still maintain a high approximation fidelity, which can translate to significant end-to-end application performance improvement.

==> tex/08-Discussion.tex <==
\section{Discussion}
In this paper, we focus on linear interferometry in the Gaussian Boson Sampling circuit, while there are several other transformations we can optimize in this system.

\textbf{Squeezing:} In our experiments on graph problems, we have already noticed that the squeezing parameters have a significant impact on the end-to-end results because it directly decides the mean photon numbers in the system. For this parameter, the usual way is to pick a scalar for the adjacency matrix of the graph and change all the squeezing gates simultaneously by multiplying the scalar\cite{bromley2020applications}. While there is no standard for setting the parameters, we believe choosing a reasonable model for squeezing can greatly improve the result accuracy.

\textbf{Displacement:} \cite{schuld2020measuring} shows how displacement can affect the final distribution of samples. While it changes the mean photon numbers in the whole system, the covariance matrices of Gaussian states are preserved. One of the future directions is to study how to add Displacement in the circuit to compensate for the gate photon loss.

\textbf{Device Architecture:} The device architecture will directly influence the decomposition strategy, in this paper, we restrict our device to a rectangular form, we believe that our method is easily extended to other device structures by first finding a standard template and fit it into real structure of the device. 
 
